Generating Custom Code for Efficient Query Execution on Heterogeneous Processors

Processor manufacturers build increasingly specialized processors to mitigate the effects of the power wall to deliver improved performance. Currently, database engines are manually optimized for each processor: A costly and error prone process. In this paper, we propose concepts to enable the database engine to perform per-processor optimization automatically. Our core idea is to create variants of generated code and to learn a fast variant for each processor. We create variants by modifying parallelization strategies, specializing data structures, and applying different code transformations. Our experimental results show that the performance of variants may diverge up to two orders of magnitude. Therefore, we need to generate custom code for each processor to achieve peak performance. We show that our approach finds a fast custom variant for multi-core CPUs, GPUs, and MICs.

==> query_ssb41.csv.tex <==


















==> simple-aggregation-query-1-medium-selectivity.csv.tex <==






















==> table_sf10_feature_wise_per_query_measurements.tex <==
\setlength{\tabcolsep}{1pt}
\begin{table*}
\begin{center}
\begin{tabular}{ | c | c | c | c | }
\hline
Query & cpu & dgpu & phi\\
\hline
query\_ssb11 &      0.167 &      0.020 &      0.180\\
query\_ssb12 &      0.100 &      0.018 &      0.062\\
query\_ssb13 &      0.098 &      0.016 &      0.069\\
query\_ssb32 &      0.203 &      0.147 &      0.173\\
query\_ssb33 &      0.115 &      0.061 &      0.106\\
query\_ssb34 &      0.116 &      0.065 &      0.130\\
query\_ssb41 &      0.541 &      0.260 &      0.546\\
query\_ssb42 &      0.413 &      0.123 &      0.361\\
query\_ssb43 &      0.194 &      0.303 &      0.366\\
tpch\_query5 &      0.754 &      0.255 &      0.676\\
tpch\_query6 &      0.168 &      0.012 &      0.034\\
\hline
\end{tabular}
\end{center}
\end{table*}



==> table_ssbm_compilation_times.tex <==

\setlength{\tabcolsep}{1pt}
\begin{table*}[t]
\begin{center}
{%\scriptsize
\begin{tabular}{ | c | c ||  c  c  c  c | c  c  c  c | c  c  c  c | c  c  c  c |  }
\hline
& Hyper &  \multicolumn{4}{c|}{Compiled for CPU} & \multicolumn{4}{c|}{Compiled for iGPU}  & \multicolumn{4}{c|}{Compiled for dGPU} & \multicolumn{4}{c|}{Compiled for MIC}\\
& (CPU) & cpu-o&igpu-o&dgpu-o&mic-o&cpu-o&igpu-o&dgpu-o&mic-o&cpu-o&igpu-o&dgpu-o&mic-o&cpu-o&igpu-o&dgpu-o&mic-o\\
\hline
%q11	q12	q13	q21	q22	q23	q31	q32	q33	q34	q41	q42	q43
%30	29	31	83	81	76	88	86	85	89	104	110	107
Q1.1&0.030&0.079&0.087&0.083&0.082&0.106&0.114&0.116&0.111&0.182&0.176&0.173&0.176&0.186&0.184&0.219&0.168\\
Q1.2&0.029&0.078&0.083&0.084&0.086&0.109&0.115&0.116&0.114&0.179&0.204&0.178&0.169&0.214&0.215&0.171&0.215\\
Q1.3&0.031&0.079&0.085&0.086&0.084&0.113&0.112&0.118&0.120&0.185&0.175&0.176&0.187&0.178&0.209&0.221&0.214\\
\hline
Q3.2&0.086&0.178&0.187&0.187&0.185&0.256&0.285&0.261&0.269&0.422&0.446&0.426&0.426&1.009&0.847&0.844&0.927\\
Q3.3&0.085&0.178&0.187&0.185&0.192&0.260&0.274&0.269&0.278&0.382&0.369&0.381&0.383&1.024&0.778&0.935&0.776\\
Q3.4&0.089&0.182&0.190&0.193&0.190&0.263&0.269&0.275&0.264&0.403&0.421&0.492&0.429&1.040&0.879&0.854&0.842\\
\hline
Q4.1&0.104&0.219&0.235&0.226&0.232&0.321&0.343&0.345&0.338&0.464&0.449&0.471&0.455&1.122&1.090&1.042&0.872\\
Q4.2&0.110&0.222&0.238&0.229&0.234&0.325&0.353&0.346&0.343&0.480&0.460&0.476&0.447&1.184&0.919&0.994&1.011\\
Q4.3&0.107&0.224&0.241&0.236&0.235&0.314&0.347&0.341&0.348&0.489&0.608&0.506&0.512&1.159&1.169&1.166&1.101\\
\hline
\hline
Q5&0.144&0.268&0.288&0.288&0.291&0.400&0.417&0.425&0.421&0.657&0.688&0.618&0.652&1.206&1.075&1.063&1.080\\
Q6&0.028&0.041&0.036&0.040&0.034&0.048&0.047&0.046&0.051&0.093&0.081&0.080&0.076&0.057&0.040&0.047&0.046\\
Q7&0.165&0.265&0.284&0.287&0.284&0.376&0.438&0.412&0.413&0.641&0.747&0.772&0.960&1.167&1.205&1.117&1.161\\
\hline
\end{tabular}
}
\end{center}
%	\caption{Execution times of variants oimized for CPU, iGPU, dGPU, and MIC for selected queries of the star schema benchmark (SF10), executed on all processors. We need custom variants per processor to achieve peak performance.}        
%\vspace{-0.2cm}
	\caption{Kernel compilation times in seconds of variants optimized for CPU, iGPU, dGPU, and MIC for selected queries of the star schema and TPC-H benchmark.}   
        \label{table:compilation_times_selected_ssb_queries}
%        \vspace{-0.4cm}
\end{table*}

